Migrating Client Code without Change Examples

API developers evolve software libraries to fix bugs, add new features, or refactor code. To benefit from such library evolution, the programmers of client projects have to repetitively upgrade their library usages and adapt their codebases to any library API breaking changes (e.g., API renaming). Such adaptive changes can be tedious and error-prone. Existing tools provide limited support to help programmers migrate client projects from old library versions to new ones. For instance, some tools extract API mappings be-tween library versions and only suggest simple adaptive changes (i.e., statement updates); other tools suggest or automate more complicated edits (e.g., statement insertions) based on user-provided exemplar code migrations. However, when new library versions are available, it is usually cumbersome and time-consuming for users to provide sufficient human-crafted samples in order to guide automatic migration. In this paper, we propose a novel approach, AutoUpdate, to further improve the state of the art. Instead of learning from change examples, we designed AutoUpdate to automate migration in a compiler-directed way. Namely, given a compilation error triggered by upgrading libraries, AutoUpdate exploits 13 migration opera-tors to generate candidate edits, and tentatively applies each edit until the error is resolved or all edits are explored. We conducted two experiments. The first experiment involves migrating 371 tutorial examples between versions of 5 popular libraries. AutoUpdate reduced migration-related compilation errors for 92.7% of tasks. It eliminated such errors for 32.4% of tasks, and 33.9% of the tasks have identical edits to manual migrations. In the second experiment, we applied AutoUpdate to migrate two real client projects of lucene. AutoUpdate successfully migrated both projects, and the migrated code passed all tests.

==> body/implementation.tex <==
\section{Implementation}
\label{sec:implementation}
Martinez and Monperrus~\cite{martinez:hal-01321615} implement an automatic-program-repair tool, called Astor. The purpose of Astor is to repair the bugs in a program. Its repair process is as follow: (1) executing a set of test cases; (2) locating the buggy lines with Gzoltar~\cite{riboira2010gzoltar} based on their execution results; (3) mutating code with repair operators; and (4) selecting a subset of mutations according to their execution results. The process continues until a mutation passes all the test cases or maximum attempts are met.

Although the purpose of Astor is different from updating client code, some underlying techniques of Astor are useful to implement \tool (\emph{e.g.}, the technique to mutate code). To reduce our implementation effort, we build our tool on the top of Astor, and extends it from the following perspectives:

\textbf{1. Compiling client code to locate its errors.} The inputs of Astor are a buggy project \emph{without compilation errors} and a set of test cases. The input of \tool is a project whose libraries are updated, and it \emph{has compilation errors}. We extend Astor to compile a project and to locate the lines with compilation errors. The underlying compiler is JDT.

\textbf{2. Mutating code to resolve compilation errors.} Although Astor provides a technique to modify programs, its repair actions are designed to repair bugs, which cannot repair compilation errors during the migration of client code. To handle the problem, we implement all the repair actions in Section~\ref{sec:approach:action}.

\textbf{3. Guiding the updating process.} Astor allows guiding the repair process under a genetic algorithm. In particular, Astor calculates the fitness value of a solution, according the number of passing and failing test cases. Our revised fitness function guides the migration process, according to the number of compilation errors.



\textbf{4. Mining API mappings.} As Astor does not provide any supports for extracting API elements and their mappings, we implement the techniques in Section~\ref{sec:approach:input} as a separate tool. From the API documents of two versions, the tool parses their HTML files to extract all the declared API elements. After that, it extracts the mappings of API types, methods, and fields. All the extracted mappings are stored in local files.

Although we reuse the framework of an automatic-program-repair tool to implement \tool, it is a novel approach with the following major differences:

\textbf{1. Automatic program repair and \tool modify code for different purposes.} A tool like Astor modifies code to repair its bugs, but \tool modifies code to resolve compilation errors that are introduced during API migration. Researchers believe that it is difficult to locate bugs~\cite{wong2016}, and even the definition of bugs is inconsistent~\cite{herzig2013s}. In the contrast, a compiler is able to precisely locate compilation errors, and their definition is less controversial.

\textbf{2. Automatic program repair and \tool have different inputs and outputs.} A tool like Astor needs many high-quality test cases to locate faults and to guide the repair process, but \tool does not need such inputs. As their outputs, a tool like Astor synthesizes code without bugs, but \tool tries to synthesize code without compilation errors, which is easier to check.


\textbf{3. Automatic program repair and \tool modify code in different ways.} Automatic program repair modifies code behaviors from buggy to correct, but \tool tries not to change code behaviors. As a result, their repair operators are different from ours, and their operators cannot update code to call newer libraries.


In summary, to reduce the development effort, instead of implementing from scratch, we build our tool on Astor. Although both the tools modify code in a similar way, \tool is a novel tool, since their purposes, inputs, outputs, and repair operators are quite different. The two tools can complement each other in real development, since code migration can introduce bugs. We further discuss this issue in Section~\ref{sec:discuss}.

